Style-based Clustering of Visual Artworks and the Play of Neural Style-Representations

Clustering artworks based on style can have many potential real-world applications like art recommendations, style-based search and retrieval, and the study of artistic style evolution of an artist or in an artwork corpus. We introduce and deliberate over the notion of 'Style-based clustering of visual artworks'. We argue that clustering artworks based on style is largely an unaddressed problem. We explore and devise different neural feature representations - from the style-classification, style-transfer to large language vision models - that can be then used for style-based clustering. Our objective is to assess the relative effectiveness of these devised style-based clustering approaches through qualitative and quantitative analysis by applying them to multiple artwork corpora and curated synthetically styled datasets. Besides providing a broad framework for style-based clustering and evaluation, our analysis provides some key novel insights on feature representations, architectures and implications for style-based clustering.

==> figures/tex_files/feat_ext.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/images/arc_figures/fnn-2.pdf}
    \caption{}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/images/arc_figures/ftext-2.pdf}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/images/arc_figures/fstylegan-2.pdf}
    \caption{}
\end{subfigure}
\hfill
\begin{subfigure}[b]{\columnwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|l}
\textbf{Visual Elements} & \textbf{Concepts} \\ \hline

Subject & Representational, Non-representational \\ \hline
Line & \begin{tabular}[c]{@{}l@{}}Blurred, Broken, Controlled, Curved, Diagonal,\\ Horizontal, Vertical, Meandering, Thick, Thin, \\Active, Energetic, Straight\end{tabular} \\ \hline
Texture & Bumpy, Flat, Smooth, Gestural, Rough \\ \hline
 Color & \begin{tabular}[c]{@{}l@{}}
 Calm, Cool, Chromatic, Monochromatic, Muted,\\ Warm, Transparent \end{tabular} \\ \hline
Shape & \begin{tabular}[c]{@{}l@{}}Ambiguous, Geometric, Amorphous, Biomorphic,\\ Closed, Open, Distorted, Heavy, Linear, Organic, \\Abstract, Decorative, Kinetic, Light\end{tabular} \\ \hline
Light and Space & \begin{tabular}[c]{@{}l@{}}Bright, Dark, Medium, Atmospheric, Planar,\\ Perspective\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}General Principles \\of Art \end{tabular} & \begin{tabular}[c]{@{}l@{}}Overlapping, Balance, Contrast, Harmony, Pattern,\\ Repetition, Rhythm, Unity, Variety, Symmetry,\\ Proportion, Parallel\end{tabular}
\end{tabular}}
    \caption{}
\end{subfigure}
    \caption{Architecture for extracting different artwork features. The first column showcases the process of extracting (a) $F_{NN}$ and (b) $F_{stylegan}$ features. The second column showcases the process of extracting (c) $F_{text}$ features and the style taxonomy used for $F_{annot}$ .}
    \label{fig:feat_ext}
\end{figure*}

==> sections/feature_exploration/nn_features.tex <==
\subsection{Neural Network based Style Features ($F_{NN}$)}
\label{sec:nn_feat}
In this subsection, we discuss the neural network based style features we have utilized with the DEC model. Neural networks (NN) have been used in previous works to extract style-based features for various style-based tasks such as style classification \cite{stclass16,stclass18}, style-transfer \cite{gatysnst}, style-based retrieval \cite{cnn-style-retrieval}, etc. We study two different types of $F_{NN}$ features for style-based clustering:  

\textbf{DenseNet Features ($F_{dense}$)}:
For the application of clustering of visual artworks, \cite{Castellano_2022} have utilized DenseNet \cite{huang2018densely} to extract features from the artworks and incorporate these features into the deep embedded clustering model (DEC) to obtain a set of clusters comprising of artworks. In their work, they have extracted $F_{dense}$ from the last layer of the DenseNet. This layer would contain all types of information pertaining to an artwork as each layer of the DenseNet is connected to all its previous layers. Their work mostly focuses on the content clustering as well as art movement and artist based clustering. In our exploration, we utilize $F_{dense}$ features to check whether these features can be utilized for style based clustering for visual artworks. Similar to \cite{Castellano_2022}, after obtaining the features for each artwork in the dimensions 1024$\times$7$\times$7, we apply global average pooling (GAP) \cite{gpa} to obtain 1024 feature vector for each artwork. 

\textbf{Convolutional Neural Network Features ($F_{CNN}$)}:
One of the pioneering works in the domain of style transfer \cite{gatysnst} observed that for a convolutional neural network, specifically for the VGG19 model, the $conv1\_1$, $conv2\_1$, $conv3\_1$, $conv4\_1$, and $conv5\_1$ layers (the first convolutional layer after pooling layer, except for $conv1\_1$), capture the style of a given image better than the rest of the layers. They have utilized the features extracted from these specific layers to achieve style-transfer. Style-transfer is the method of transferring the "style" from a style reference image into a content image. 

Works such as \cite{stclass16,stclass18} have utilized the style features introduced by \cite{gatysnst} for style classification of artworks. In their work, they explore different combinations of features extracted from differen layers of the CNN as well as different mathematical correlations and combinations of these features for style classification. They observe that the gram matrices of features obtained from $conv5\_1$ ($F_{gram}$) yield one of the best results in the task of classification. They also observe that the dot product of $F_{gram}$ and cosine similarity of the features extracted from $conv5\_1$ ($F_{g \cdot c}$) also produces good results. In our work, we utilize $F_{gram}$ and $F_{g \cdot c}$ and explore their impact on unsupervised style-based clustering. We reduce the dimensions of $F_{gram}$ and $F_{g \cdot c}$ from 512$\times$512 to 512 for each artwork by utilizing GAP. The architecture for extracting $F_{NN}$ features can be seen in Figure \ref{fig:feat_ext} (a).

% We consider different correlations of these style features for style-based clustering:
% \begin{enumerate}
%     \item \textbf{Gram based correlation between CNN features ($F_{gram}$)}: We extract features from each style layer of VGG-19 ($conv1\_1$, $conv2\_1$, $conv3\_1$, $conv4\_1$, and '$conv5\_1$') individually for a given artwork and calculate the gram matrices of these features. The gram matrix between two feature maps $F^{(i)}$ and $F^{(j)}$ is defined as 
% \begin{equation}
%     Gram_{ij} = F^{(i)} \cdot F^{(j)}
% \end{equation}
% where $Gram_{ij}$ is the inner product between $F^{(i)}$ and $F^{(j)}$.  
%     \item \textbf{Mathematical correlations between CNN features ($F_{corr}$)}: We calculate different mathematical correlations between the features maps extracted from a each style layer. We describe each correlation in detail later in this subsection.  
%     \item \textbf{Correlation between correlations of each layer}: We consider the correlations between the correlations calculated on CNN features extracted from each layer (Gram matrices, etc.). 
% \end{enumerate}

% \textbf{Mathematical Correlations for CNN features ($F_{corr}$)}: Similar to \cite{stclass16,stclass18}, We consider different correlations between the CNN features to utilize them for achieving style-based clustering of artworks. To describe these correlation metrics in mathematics, we take feature maps extracted from ’conv5\_1’ as the main example. For a 224x224 image, we obtain 512 feature maps with each feature map having a dimension of 14x14. Each feature map is
% therefore vectorized into a 14 × 14 = 196-dimensional vector. The 196 values of a feature map can be viewed as values generated
% based on a random variable, and the $i$th feature map and the
% $j$th feature map can be represented by two 196-dimensional
% vectors $F^{(i)}= \{f^{(i)}_{1},....,f^{(i)}_{196}\}$ and $F^{(j)}= \{f^{(j)}_{1},...., f^{(j)}_{196}\}$ respectively. 
% \begin{enumerate}
%     \item \textbf{Euclidean Distance}: The Euclidean distance ($ed_{ij}$) between two features maps $F^{(i)}$ and $F^{(j)}$ is defined as 
%     \begin{equation}
%         ed_{ij} = \sqrt{\sum_{k=1}^{196}(f^{(i)}_{k} - f^{(j)}_{k})}
%     \end{equation}
%     \item \textbf{Pearson Correlation}: The Pearson correlation coefficient ($\rho_{ij}$) between two features maps $F^{(i)}$ and $F^{(j)}$ is defined as 
%     \begin{equation}
%         \rho_{ij} = \frac{[(f^{(i)} - \bar{f}^{(i)})(f^{(i)} - \bar{f}^{(i)})]}{\sigma^{(i)} \sigma^{(j)}}
%     \end{equation}
%     where $\bar{f}^{i}$ and $\bar{f}^{j}$ are the means of $F^{i}$ and $F^{j}$,  respectively and $\sigma^{i}$ and $\sigma^{j}$ are the standard deviations of $F^{i}$ and $F^{j}$, respectively. 
%     \item \textbf{Spearman Correlation}: The Spearman correlation coefficient ($r_{ij}$) is the Pearson correlation coefficient between ranked variables. Therefore, the value $r_{ij}$ between two features maps $F^{(i)}$ and $F^{(j)}$ is defined as 
%     \begin{equation}
%         r_{ij} = \frac{[(g^{(i)} - \bar{g}^{(i)})(g^{(i)} - \bar{g}^{(i)})]}{\sigma^{(i)}_{g} \sigma^{(j)}_{g}}
%     \end{equation}
%     where $\bar{g}^{(i)}$ and $\bar{f}^{(i)}$ are the means of sorted $F^{(i)}$ and sorted $F^{(j)}$,  respectively and $\sigma^{(i)}_{g}$ and $\sigma^{j}_{(g)}$ are the standard deviations of sorted $F^{(i)}$ and sorted $F^{(j)}$, respectively.
%     \item \textbf{Covariance}: The covariance $cov_{ij}$ between two features maps $F^{(i)}$ and $F^{(j)}$ is defined as 
%     \begin{equation}
%         cov_{ij}=[(f^{(i)} - \bar{f}^{(i)})(f^{(i)} - \bar{f}^{(i)})]
%     \end{equation}
%     \item \textbf{Chebychev distance}: The Chebychev distance ($v_{ij}$) between two features maps $F^{(i)}$ and $F^{(j)}$ is defined as 
% \begin{equation}
%     v_{ij}= \lim_{k \to \infty} (\sum_{k=1}^{196}\|f^{(i)}_{k} - f^{(j)}_{k}\|^k)^{1/k}
% \end{equation}
% which is also known as the $L_{\infty}$ norm between feature maps $F^{(i)}$ and $F^{(j)}$.
%     \item \textbf{Cosine Similarity}: The Cosine similarity ($s{ij}$) between two feature maps $F^{(i)}$ and $F^{(j)}$ is defined as
%     \begin{equation}
%         s_{ij}= \frac{F^{(i)} \cdot F^{(j)}}{\|F^{(i)}\|\|F^{(j)}\|}
%     \end{equation}
%     where $F^{(i)} \cdot F^{(j)}$ signifies the inner product of $F^{(i)}$ and $F^{(j)}$.
% \end{enumerate}

% The calculation for correlations is done for all pairs of feature maps. For $'conv5\_1'$ layer which outputs 512 feature maps for a given artwork, 512 x 512 correlation values can be obtained. We utilize all the different types of correlations mentioned above in Section \ref{sec: experiments} on different datasets to achieve style-based clustering. We reduce the dimensions of the features using global pooling average.

==> sections/feature_exploration/stylegan_features.tex <==
\subsection{StyleGan based Style Features ($F_{stylegan}$)}
\label{sec:stylegan_feat}
In this subsection, we discuss the different stylegan features utilized in \cite{stylegan} to train a generative adversarial network (GAN) \cite{GAN} to capture the different types of style information present in an image. Their work primarily focuses on realistic images. In their work, 
they have modified GAN to incorporate a style input at different convolutional layers to drive the GAN model to generate images in specific styles. They have divided the 7 blocks layers present in the synthesis network into three levels based on the style aspects captured by each layer for face images as follow: 
\begin{enumerate}
    \item \textbf{Coarse-grained style ($F_{coarse}$)}: The first two blocks of the synthesis network (4$\times$4, 8$\times$8) capture the coarse level information present in an image such as pose, general hair style, face shape, eyeglasses, etc. 
    \item \textbf{Middle-grained style ($F_{middle}$)}: The third and fourth block of the synthesis network (16$\times$16, 32$\times$32) capture the middle level information present in an image such as facial features, eyes open or closed, etc.
    \item \textbf{Fine-grained style ($F_{fine}$)}: The fifth, sixth and seventh block of the synthesis network (64$\times$64, 128$\times$128, 256$\times$256) capture the fine-grained level style information such as color scheme and micro-structure.
\end{enumerate}

In their experiment, the authors have experimented purely on photo-realistic images. In our work, we experiment with stylegan for artworks, we extract the style features from the transformers present in each block of the synthesis network. We categorize the extracted features based on the different styles described above and concatenate them column wise. The dimension of the features for each artwork is 1536, 2048, and 1344 for $F_{coarse}$, $F_{middle}$ and $F_{fine}$ respectively. We experiment with each category of these features to achieve style-based clustering. The architecture for extracting $F_{stylegan}$ features can be seen in Figure \ref{fig:feat_ext} (b).

==> sections/feature_exploration/text_features.tex <==
\subsection{Textual Style Features ($F_{text}$)}
\label{sec:text_feat}
In this subsection, we discuss in detail our two proposed approaches for style based clustering that explicitly factor in the artistic style information from the artworks through text. The architecture for extracting $F_{text}$ features can be seen in Figure \ref{fig:feat_ext} (c). %Later we discuss an improvement of the cluster initialization method where the number of clusters is dynamically determined. (section \ref{sec:dynamic_cluster}).

\subsubsection{Artwork caption representation ($F_{caption}$)}
\label{sec: caption}
In this approach, we generate the artwork representation using the text description of the artwork. The text description of the artwork encloses the content as well as the coarse-grained style information. %In  Figure \ref{fig: caption_example}, we present example artworks along with the text description. 
The coarse-grained style information in the text description is depicted with the keywords such as painting, drawing, portrait, etc.  Formally, we obtain $F_{caption}$ for an artwork $a_i$ as:

\begin{equation}
    F_{caption} = T(C(a_i))
\end{equation}

where $C$ is the caption generator and $T$ is the text encoder to encode the caption for the artwork $a_i$.

In this work, we use the \textit{Bootstrapping Language-Image Pre-training for Unified Vision} (BLIP) \cite{li2022blip} model as the caption generator ($C$) for artworks. Specifically, we use the BLIP Image Captioning Large model which uses the BERT \cite{devlin2018bert} model as the text encoder and the ViT-L \cite{dosovitskiy2021image}  model as the vision backbone. It has been trained on 129 Million images from the COCO, VG, CC, SBU, and LAION datasets. The BLIP model takes in the input artwork and gives us an output text that describes the artwork in a sentence (see Figure \ref{fig: caption_example}). 
% These descriptions alleviate the need to rely on the DenseNet model to learn the visual features. 
Next, we use sentence-transformer \cite{reimers2019sentencebert} as the text encoder ($T$) for artwork captions. We obtain a 384-dimensional artwork representation $F_{caption}$ for each artwork. We then use these artwork representation $F_{caption}$ as input artwork features in the DEC model. It is to be noted that we use BLIP captioning model and sentence transformer as a proxy for $C$ and $T$ and it could be replaced with other image captioning and text encoder models.

%\input{figures/tex_files/caption_example}

\subsubsection{Artwork style concept annotation representation ($F_{annot}$)}
\label{sec: annotation}
In this approach, we annotate artworks with style concepts based on the fundamental principles of art \cite{ocvirk1968art}. A set of 59 different concepts across seven visual elements has been utilized by \cite{8334453} in their work (see Table \ref{tab: principles}). Formally, we obtain the artwork representation for an artwork $a_i$ with style concept annotation as:

\begin{equation}
    F_{annot} = T(S(a_i, taxonomy, instruction)
\end{equation}

where, $S$ is the style concept annotator and $T$ is the text encoder to encode the style concepts of an artwork. The style concept annotator considers the \textit{taxonomy} given in Table \ref{tab: principles} and the \textit{instruction} is to associate the style concepts (for each visual elements) from the taxonomy to a given artwork $a_i$.

In this work, we leverage Large Language and Vision Assistant (LLaVA) 1.5 model \cite{liu2023visual} as a style concept annotator ($S$). It is a large multi-modal model that combines the CLIP ViT-L \cite{clip} vision encoder and the Vicuna 1.5 13B text encoder fine-tuned from the LLaMA model \cite{touvron2023llama}. LLaVa can be used for general-purpose visual and language understanding tasks where given an image and a query, the model is able to answer the given query based on the image. We use sentence-transformer \cite{reimers2019sentencebert} as the text encoder ($T$) to obtain the 384 dimensional representation $F_{annot}$ for each artwork.

%Figure \ref{fig: annotation_example} depicts artworks with its respective style concept annotation with the LLaVA model. %In contrast to artwork caption (refer Figure \ref{fig: caption_example}), 
The style information available with this method is fine-grained across various artistic style dimensions. It is to be noted that we use LLaVA and sentence-transformer as a proxy and it could be replaced with other style concept annotators and text encoders respectively. 

\input{tables/principles_of_art}

%\input{figures/tex_files/style_annotation_example}

==> tables/observation_tables/dec_cluster_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[!h]
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Edvard Munch \\ Archive\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Brueghel\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Clip Illustrations\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mixed Curated\\ Dataset\end{tabular}}} \\ \cline{3-12} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{\textbf{SC}} &
  \textbf{CHI} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.547}} &
  {\color[HTML]{000000} 1425.69} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.391}} &
  {\color[HTML]{000000} 479.6} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.351}} &
  {\color[HTML]{000000} 584.72} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.31}} &
  {\color[HTML]{000000} 455.41} &
  \multicolumn{1}{c|}{0.404} &
  523.71 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.276}} &
  {\color[HTML]{000000} 828.18} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.276}} &
  {\color[HTML]{000000} 1458.85} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.237}} &
  {\color[HTML]{000000} 447.59} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.18}} &
  {\color[HTML]{000000} 657.55} &
  \multicolumn{1}{c|}{0.344} &
  1005.35 \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.554}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 3574.71} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.532}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 5254.83} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.55}} &
  {\color[HTML]{000000} 3655.1} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.555}} &
  {\color[HTML]{000000} 2966.18} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}1} &
  144.22 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.818}} &
  {\color[HTML]{000000} 778.57} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.805}} &
  {\color[HTML]{000000} 1727.47} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.827}} &
  {\color[HTML]{000000} 2072.85} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.762}} &
  {\color[HTML]{000000} 514.55} &
  \multicolumn{1}{c|}{0.513} &
  550.75 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.179}} &
  {\color[HTML]{000000} 110.85} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.226}} &
  {\color[HTML]{000000} 31.16} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.191}} &
  {\color[HTML]{000000} 92.27} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.125}} &
  {\color[HTML]{000000} 172.7} &
  \multicolumn{1}{c|}{0.396} &
  452.97 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.136}} &
  {\color[HTML]{000000} 820.54} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.194}} &
  {\color[HTML]{000000} 993.13} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.877}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 4516.36} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.39}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 4601.97} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}0.624} &
  \cellcolor[HTML]{F2CEEF}2869.02 \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.092}} &
  {\color[HTML]{000000} 665.05} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.041}} &
  {\color[HTML]{000000} 554.35} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.087}} &
  {\color[HTML]{000000} 757.6} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.07}} &
  {\color[HTML]{000000} 315.51} &
  \multicolumn{1}{c|}{-0.133} &
  1249.7 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.98}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 80216.63} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.826}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 330895.74} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.876}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 37836.54} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.862}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 2164268.51} &
  \multicolumn{1}{c|}{0.403} &
  \cellcolor[HTML]{C0F1C8}5349.69 \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.988}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 55749.82} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.99}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 75071.11} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.981}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 23309.98} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.932}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 4651.21} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}0.948} &
  \cellcolor[HTML]{CAEDFB}21290.56
\end{tabular}%
}
\caption{SC and CHI metric scores for the \textbf{synthetically curated datasets} for all features using the \textbf{DEC}. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric. The curated dataset is synthesized using \textbf{10 style images} and \textbf{50 content images}.}
\label{tab:dec_cluster_comp}
\end{table*}

==> tables/observation_tables/dec_gt_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{CHI}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  \multicolumn{2}{c}{{\color[HTML]{000000} \textbf{V-Mes}}} \\ \cline{3-10} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.404}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.938} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 523.71}} &
  {\color[HTML]{000000} 36714.5} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.349}} &
  {\color[HTML]{000000} 0.0004} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.573}} &
  {\color[HTML]{000000} 0.055} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.344}} &
  {\color[HTML]{000000} 0.861} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 1005.35}} &
  {\color[HTML]{000000} 6552.82} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.501}} &
  {\color[HTML]{000000} -0.0006} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.799}} &
  {\color[HTML]{000000} 0.052} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 1}} &
  {\color[HTML]{000000} 0.527} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 144.22}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 26406.94} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.002}} &
  {\color[HTML]{000000} -0.0002} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.011}} &
  {\color[HTML]{000000} 0.051} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.513}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.926} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 550.75}} &
  {\color[HTML]{000000} 16543.47} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.373}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.037} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.656}} &
  {\color[HTML]{000000} 0.15} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.396}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.911} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 452.97}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 17770.75} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.032}} &
  {\color[HTML]{000000} -0.014} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.21}} &
  {\color[HTML]{000000} 0.054} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.624}} &
  {\color[HTML]{000000} 0.649} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 2869.02}} &
  {\color[HTML]{000000} 6336.87} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.018}} &
  {\color[HTML]{000000} 0.0006} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.178}} &
  {\color[HTML]{000000} 0.055} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.133}} &
  {\color[HTML]{000000} 0.014} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 1249.7}} &
  {\color[HTML]{000000} 705.66} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.005}} &
  {\color[HTML]{000000} 0.0003} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.145}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.058} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.403}} &
  {\color[HTML]{000000} 0.686} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 5349.69}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 84635.96} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.251}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.153} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.541}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.352} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.948}} &
  {\color[HTML]{000000} 0.899} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 21290.56}} &
  {\color[HTML]{000000} 15069.18} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.171}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.091} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.449}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.286}
\end{tabular}%
}
\caption{Quantitative metric scores for the mixed curated dataset as well as the art movement labelled WikiArt subset dataset for all features with \textbf{DEC}. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric.}
\label{tab:dec_gt_comp}
\end{table*}

==> tables/observation_tables/dec_style_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[!h]
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Edvard Munch \\ Archive\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Brueghel\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Clip Illustrations\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mixed Curated\\ Dataset\end{tabular}}} \\ \cline{3-12} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{\textbf{ARI}} &
  \textbf{V-Mes} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.498}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.724} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.492}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.698} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.463}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.692} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.461}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.63} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}0.349} &
  \cellcolor[HTML]{F2CEEF}0.573 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.554}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.762} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.58}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.792} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.634}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.817} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.371}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.589} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}0.501} &
  \cellcolor[HTML]{CAEDFB}0.799 \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.191}} &
  {\color[HTML]{000000} 0.362} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.185}} &
  {\color[HTML]{000000} 0.419} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.191}} &
  {\color[HTML]{000000} 0.394} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.107}} &
  {\color[HTML]{000000} 0.263} &
  \multicolumn{1}{c|}{0.002} &
  0.011 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.41}} &
  {\color[HTML]{000000} 0.543} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.57}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.669} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.405}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.532} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.145}} &
  {\color[HTML]{000000} 0.321} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}0.403} &
  \cellcolor[HTML]{C0F1C8}0.67 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.021}} &
  {\color[HTML]{000000} 0.088} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.006}} &
  {\color[HTML]{000000} 0.052} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.025}} &
  {\color[HTML]{000000} 0.104} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.013}} &
  {\color[HTML]{000000} 0.072} &
  \multicolumn{1}{c|}{0.032} &
  0.21 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.013}} &
  {\color[HTML]{000000} 0.081} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.007}} &
  {\color[HTML]{000000} 0.055} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.013}} &
  {\color[HTML]{000000} 0.077} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.002}} &
  {\color[HTML]{000000} 0.048} &
  \multicolumn{1}{c|}{0.018} &
  0.178 \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.015}} &
  {\color[HTML]{000000} 0.081} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.007}} &
  {\color[HTML]{000000} 0.052} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.017}} &
  {\color[HTML]{000000} 0.083} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.003}} &
  {\color[HTML]{000000} 0.056} &
  \multicolumn{1}{c|}{0.005} &
  0.145 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.303}} &
  {\color[HTML]{000000} 0.441} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.128}} &
  {\color[HTML]{000000} 0.237} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.203}} &
  {\color[HTML]{000000} 0.333} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.092}} &
  {\color[HTML]{000000} 0.186} &
  \multicolumn{1}{c|}{0.251} &
  0.541 \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.399}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.549} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.331}} &
  {\color[HTML]{000000} 0.464} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.366}} &
  {\color[HTML]{000000} 0.511} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.258}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.371} &
  \multicolumn{1}{c|}{0.171} &
  0.449
\end{tabular}%
}
\caption{ARI and V-Mes metric scores for the \textbf{synthetically curated datasets} for all features using \textbf{DEC}. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric. The curated dataset is synthesized using \textbf{10 style images} and \textbf{50 content images}.}
\label{tab:dec_style_comp}
\end{table*}

==> tables/observation_tables/k_cluster_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[!h]
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Edvard Munch \\ Archive\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Brueghel\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Clip Illustrations\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mixed Curated\\ Dataset\end{tabular}}} \\ \cline{3-12} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  {\color[HTML]{000000} \textbf{CHI}} &
  \multicolumn{1}{c|}{\textbf{SC}} &
  \textbf{CHI} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.101}} &
  {\color[HTML]{000000} 18.49} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.098}} &
  {\color[HTML]{000000} 19.44} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.09}} &
  {\color[HTML]{000000} 19.12} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.07}} &
  {\color[HTML]{000000} 16.73} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}0.073} &
  21.37 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.282}} &
  {\color[HTML]{000000} 105.2} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.221}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 136.26} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.282}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 113.88} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.193}} &
  {\color[HTML]{000000} 67.8} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}0.183} &
  \cellcolor[HTML]{C0F1C8}142.15 \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.447}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 2548.54} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.456}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 4060.88} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.479}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 2898.03} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.454}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 2200.79} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}0.29} &
  \cellcolor[HTML]{CAEDFB}13468.88 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.008}} &
  {\color[HTML]{000000} 6.26} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.02}} &
  {\color[HTML]{000000} 7.94} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.01}} &
  {\color[HTML]{000000} 6.61} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.016}} &
  {\color[HTML]{000000} 6.43} &
  \multicolumn{1}{c|}{-0.017} &
  8.016 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.045}} &
  {\color[HTML]{000000} 24.53} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.047}} &
  {\color[HTML]{000000} 22.6} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.047}} &
  {\color[HTML]{000000} 25.02} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.042}} &
  {\color[HTML]{000000} 22.98} &
  \multicolumn{1}{c|}{0.03} &
  30.68 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.049}} &
  {\color[HTML]{000000} 36.96} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.055}} &
  {\color[HTML]{000000} 32.14} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.06}} &
  {\color[HTML]{000000} 36.53} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.052}} &
  {\color[HTML]{000000} 34.86} &
  \multicolumn{1}{c|}{0.034} &
  44.58 \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.097}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 113.99} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.091}} &
  {\color[HTML]{000000} 94.31} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.095}} &
  {\color[HTML]{000000} 113.74} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.097}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 105.97} &
  \multicolumn{1}{c|}{0.051} &
  \cellcolor[HTML]{F2CEEF}129.7 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.047}} &
  {\color[HTML]{000000} 17.91} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.055}} &
  {\color[HTML]{000000} 15.79} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.05}} &
  {\color[HTML]{000000} 18.31} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.069}} &
  {\color[HTML]{000000} 16.18} &
  \multicolumn{1}{c|}{0.041} &
  20.69 \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.328}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 181.16} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.403}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 148.56} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.331}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 233.01} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.384}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 141.39} &
  \multicolumn{1}{c|}{0.031} &
  22.56
\end{tabular}%
}
\caption{SC and CHI metric scores for the \textbf{synthetically curated datasets} for all features using the \textbf{K-Means}. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric. The curated dataset is synthesized using \textbf{10 style images} and \textbf{50 content images}.}
\label{tab:k_cluster_comp}
\end{table*}

==> tables/observation_tables/k_gt_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{CHI}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  \multicolumn{2}{c}{{\color[HTML]{000000} \textbf{V-Mes}}} \\ \cline{3-10} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mixed\\ Curated\end{tabular}}}} &
  {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Subset\end{tabular}}} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.073}} &
  {\color[HTML]{000000} 0.018} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 21.37}} &
  {\color[HTML]{000000} 20.49} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.543}} &
  {\color[HTML]{000000} -0.0002} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.675}} &
  {\color[HTML]{000000} 0.054} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.183}} &
  {\color[HTML]{000000} 0.036} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 142.15}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 90.1} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.743}} &
  {\color[HTML]{000000} -0.0007} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.828}} &
  {\color[HTML]{000000} 0.051} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.29}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.435} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 13468.88}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 18712.64} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.073}} &
  {\color[HTML]{000000} -0.0004} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.351}} &
  {\color[HTML]{000000} 0.05} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.017}} &
  {\color[HTML]{000000} -0.0018} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 8.016}} &
  {\color[HTML]{000000} 6.14} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.403}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.04} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.67}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.15} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.03}} &
  {\color[HTML]{000000} 0.03} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 30.68}} &
  {\color[HTML]{000000} 40.15} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.023}} &
  {\color[HTML]{000000} -0.0009} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.204}} &
  {\color[HTML]{000000} 0.048} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.034}} &
  {\color[HTML]{000000} 0.036} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 44.58}} &
  {\color[HTML]{000000} 58.23} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.024}} &
  {\color[HTML]{000000} 0.0011} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.206}} &
  {\color[HTML]{000000} 0.058} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.051}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.055} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 129.7}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 176.62} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.015}} &
  {\color[HTML]{000000} 0.0009} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.182}} &
  {\color[HTML]{000000} 0.057} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.041}} &
  {\color[HTML]{000000} 0.035} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 20.69}} &
  {\color[HTML]{000000} 33.86} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.322}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.12} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.562}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.34} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.031}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.038} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 22.56}} &
  {\color[HTML]{000000} 47.32} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.209}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.113} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.472}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.313}
\end{tabular}%
}
\caption{Quantitative metric scores for the mixed curated dataset as well as the art movement labelled WikiArt subset dataset for all features with \textbf{K-Means}. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric.}
\label{tab:k_gt_comp}
\end{table*}

==> tables/observation_tables/k_style_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[!h]
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Edvard Munch \\ Archive\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}WikiArt\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Brueghel\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Clip Illustrations\\ Dataset\end{tabular}}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mixed Curated\\ Dataset\end{tabular}}} \\ \cline{3-12} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  {\color[HTML]{000000} \textbf{V-Mes}} &
  \multicolumn{1}{c|}{\textbf{ARI}} &
  \textbf{V-Mes} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.601}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.615} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.511}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.719} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.689}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.723} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.433}} &
  {\color[HTML]{000000} 0.457} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}0.543} &
  \cellcolor[HTML]{C0F1C8}0.675 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 1}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 1} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.995}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.995} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.991}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.991} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.65}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.74} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}0.743} &
  \cellcolor[HTML]{CAEDFB}0.828 \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.192}} &
  {\color[HTML]{000000} 0.363} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.186}} &
  {\color[HTML]{000000} 0.419} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.18}} &
  {\color[HTML]{000000} 0.397} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.1074}} &
  {\color[HTML]{000000} 0.263} &
  \multicolumn{1}{c|}{0.073} &
  0.351 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.65}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.79} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.88}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.9} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.52}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.68} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.34}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.48} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}0.403} &
  \cellcolor[HTML]{F2CEEF}0.67 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.052}} &
  {\color[HTML]{000000} 0.13} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.052}} &
  {\color[HTML]{000000} 0.121} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.04}} &
  {\color[HTML]{000000} 0.115} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.034}} &
  {\color[HTML]{000000} 0.104} &
  \multicolumn{1}{c|}{0.023} &
  0.204 \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.035}} &
  {\color[HTML]{000000} 0.116} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.027}} &
  {\color[HTML]{000000} 0.09} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.048}} &
  {\color[HTML]{000000} 0.124} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.038}} &
  {\color[HTML]{000000} 0.111} &
  \multicolumn{1}{c|}{0.024} &
  0.206 \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.021}} &
  {\color[HTML]{000000} 0.091} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.023}} &
  {\color[HTML]{000000} 0.091} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.038}} &
  {\color[HTML]{000000} 0.12} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.008}} &
  {\color[HTML]{000000} 0.062} &
  \multicolumn{1}{c|}{0.015} &
  0.182 \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.466}} &
  {\color[HTML]{000000} 0.581} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.513}} &
  {\color[HTML]{000000} 0.546} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.403}} &
  {\color[HTML]{000000} 0.546} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.543}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.653} &
  \multicolumn{1}{c|}{0.322} &
  0.562 \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.422}} &
  {\color[HTML]{000000} 0.563} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.299}} &
  {\color[HTML]{000000} 0.446} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.35}} &
  {\color[HTML]{000000} 0.497} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.311}} &
  {\color[HTML]{000000} 0.411} &
  \multicolumn{1}{c|}{0.209} &
  0.472
\end{tabular}%
}
\caption{ARI and V-Mes metric scores for the \textbf{synthetically curated datasets} for all features using \textbf{K-Means}. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric. The curated dataset is synthesized using \textbf{10 style images} and \textbf{50 content images}.}
\label{tab:k_style_comp}
\end{table*}

==> tables/observation_tables/mix_k_dec.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{CHI}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  \multicolumn{2}{c}{{\color[HTML]{000000} \textbf{V-Mes}}} \\ \cline{3-10} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.073}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.404} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 21.37}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 523.71} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.543}} &
  {\color[HTML]{000000} 0.349} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.675}} &
  {\color[HTML]{000000} 0.573} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.183}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.344} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 142.15}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 1005.35} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.743}} &
  {\color[HTML]{000000} 0.501} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.828}} &
  {\color[HTML]{000000} 0.799} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.29}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000}0.563} &
  \multicolumn{1}{c|}{\color[HTML]{000000} 13468.88} &
  {\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 37891.34}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.073}} &
  {\color[HTML]{000000} 0.002} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.351}} &
  {\color[HTML]{000000} 0.011} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.017}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.513} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 8.016}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 550.75} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.403}} &
  {\color[HTML]{000000} 0.373} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.67}} &
  {\color[HTML]{000000} 0.656} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.03}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.396} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 30.68}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 452.97} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.023}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.032} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.204}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.21} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.034}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.624} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 44.58}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 2869.02} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.024}} &
  {\color[HTML]{000000} 0.018} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.206}} &
  {\color[HTML]{000000} 0.178} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.051}} &
  {\color[HTML]{000000} -0.133} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 129.7}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 1249.7} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.015}} &
  {\color[HTML]{000000} 0.005} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.182}} &
  {\color[HTML]{000000} 0.145} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.041}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.403} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 20.69}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 5349.69} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.322}} &
  {\color[HTML]{000000} 0.251} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.562}} &
  {\color[HTML]{000000} 0.541} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.031}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.948} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 22.56}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 21290.56} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.209}} &
  {\color[HTML]{000000} 0.171} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.472}} &
  {\color[HTML]{000000} 0.449}
\end{tabular}%
}
\caption{Metrics scores for the \textbf{Mixed curated} dataset for all features for both K-Means and DEC model. The \colorbox[HTML]{CAEDFB}{highlighted} values indicate which model performs better for a feature on that specific metric. The mixed curated dataset contains \textbf{2000} images and \textbf{40} different styles.}
\label{tab:mix_k_dec}
\end{table*}



==> tables/observation_tables/mixed_curated_quant.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|ccc|ccc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{V-Mes}}} &
  \multicolumn{3}{c|}{\textbf{SC}} &
  \multicolumn{3}{c}{\textbf{CHI}} \\ \cline{3-12} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{\textbf{Base}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{\textbf{Base}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.543}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.349} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.675}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.573} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}0.077} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.073}} &
  {\color[HTML]{000000} 0.404} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}21.49} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 21.37}} &
  {\color[HTML]{000000} 523.71} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.743}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.501} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.828}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.799} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}0.208} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.183}} &
  {\color[HTML]{000000} 0.344} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}127.14} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 142.15}} &
  {\color[HTML]{000000} 1005.35} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.073}} &
  {\color[HTML]{000000} 0.002} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.351}} &
  {\color[HTML]{000000} 0.011} &
  \multicolumn{1}{c|}{-0.248} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.29}} &
  {\color[HTML]{000000} 0.563} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}359.09} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 13468.88}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 37891.34} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.414}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.414} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.707}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.682} &
  \multicolumn{1}{c|}{-0.03} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.016}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.937} &
  \multicolumn{1}{c|}{9.01} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 9.84}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 21676.54} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.025}} &
  {\color[HTML]{000000} 0.019} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.21}} &
  {\color[HTML]{000000} 0.187} &
  \multicolumn{1}{c|}{-0.042} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.1}} &
  {\color[HTML]{000000} 0.911} &
  \multicolumn{1}{c|}{7.64} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 47.89}} &
  {\color[HTML]{000000} 12202.8} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.014}} &
  {\color[HTML]{000000} 0.011} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.179}} &
  {\color[HTML]{000000} 0.164} &
  \multicolumn{1}{c|}{-0.05} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.113}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.921} &
  \multicolumn{1}{c|}{8.03} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 59.98}} &
  {\color[HTML]{000000} 17621.11} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.013}} &
  {\color[HTML]{000000} 0.009} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.174}} &
  {\color[HTML]{000000} 0.152} &
  \multicolumn{1}{c|}{-0.082} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.128}} &
  {\color[HTML]{000000} 0.891} &
  \multicolumn{1}{c|}{6.988} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 134.12}} &
  {\color[HTML]{000000} 11399.32} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.322}} &
  {\color[HTML]{000000} 0.251} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.562}} &
  {\color[HTML]{000000} 0.541} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}0.015} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.041}} &
  {\color[HTML]{000000} 0.403} &
  \multicolumn{1}{c|}{16.08} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 20.69}} &
  {\color[HTML]{000000} 5349.69} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.209}} &
  {\color[HTML]{000000} 0.171} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.472}} &
  {\color[HTML]{000000} 0.449} &
  \multicolumn{1}{c|}{-0.003} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.031}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.948} &
  \multicolumn{1}{c|}{15.56} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 22.56}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 21290.56}
\end{tabular}%
}
\caption{Metrics scores for the \textbf{Mixed curated} dataset for all features for both K-Means and DEC model. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric. The mixed curated dataset contains \textbf{2000} images and \textbf{40} different styles.}
\label{tab:mix_quant}
\end{table*}

==> tables/observation_tables/wikiart_k_dec.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{SC}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{CHI}}} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  \multicolumn{2}{c}{{\color[HTML]{000000} \textbf{V-Mes}}} \\ \cline{3-10} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.018}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.938} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 20.49}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 36714.5} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0002}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.0004} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.054}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.055} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.036}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.861} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 90.1}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 6552.82} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0007}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} -0.0006} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.051}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.052} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.435}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.527} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 18712.64}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 26406.94} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0004}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} -0.0002} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.05}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.051} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0018}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.926} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 6.14}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 16543.47} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.15}} &
  {\color[HTML]{000000} 0.037} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.04}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.15} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.03}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.911} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 40.15}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 17770.75} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} -0.0009}} &
  {\color[HTML]{000000} -9.149} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.048}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.054} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.036}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.649} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 58.23}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 6336.87} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.0011}} &
  {\color[HTML]{000000} 0.0006} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.058}} &
  {\color[HTML]{000000} 0.055} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.055}} &
  {\color[HTML]{000000} 0.014} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 176.62}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 705.66} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.0009}} &
  {\color[HTML]{000000} 0.0003} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.057}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.058} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.035}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.686} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 33.86}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 84635.96} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.12}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.153} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.34}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.352} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.038}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.899} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 47.32}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 15069.18} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.113}} &
  {\color[HTML]{000000} 0.091} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.313}} &
  {\color[HTML]{000000} 0.286}
\end{tabular}%
}
\caption{Metrics scores for the \textbf{WikiArt subset} dataset for all features for both K-Means and DEC model. The \colorbox[HTML]{CAEDFB}{highlighted} values indicate which model performs better for a feature on that specific metric. The WikiArt subset dataset contains \textbf{2082} artworks with \textbf{27} art movements.}
\label{tab:wiki_k_dec}
\end{table*}

==> tables/observation_tables/wikiart_subset_quant.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }} &
  \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{ARI}}} &
  \multicolumn{2}{c}{{\color[HTML]{000000} \textbf{V-Mes}}} \\ \cline{3-6} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}} &
  {\color[HTML]{000000} \textbf{DEC}} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{dense}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0002}} &
  {\color[HTML]{000000} 0.0004} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.054}} &
  {\color[HTML]{000000} 0.055} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{gram}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0007}} &
  {\color[HTML]{000000} -0.0006} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.051}} &
  {\color[HTML]{000000} 0.052} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{NN}$}}} &
  {\color[HTML]{000000} $F_{g \cdot c}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0004}} &
  {\color[HTML]{000000} -0.0002} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.05}} &
  {\color[HTML]{000000} 0.051} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{wvec}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.04}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.037} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.15}} &
  {\color[HTML]{000000} 0.15} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{coarse}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} -0.0009}} &
  {\color[HTML]{000000} -0.014} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.048}} &
  {\color[HTML]{000000} 0.054} \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{middle}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.0011}} &
  {\color[HTML]{000000} 0.0006} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.058}} &
  {\color[HTML]{000000} 0.055} \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} &
  {\color[HTML]{000000} $F_{fine}$} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.0009}} &
  {\color[HTML]{000000} 0.0003} &
  \multicolumn{1}{c|}{{\color[HTML]{000000} 0.057}} &
  \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.058} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} $F_{caption}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.12}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.153} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.34}} &
  \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.352} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}} &
  {\color[HTML]{000000} $F_{annot}$} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.113}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.091} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.313}} &
  \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.286}
\end{tabular}%
}
\caption{Metrics scores for the \textbf{WikiArt subset} dataset for all features for both K-Means and DEC model. The \colorbox[HTML]{CAEDFB}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{F2CEEF}{third best} results are highlighted for each metric. The WikiArt subset dataset contains \textbf{2082} artworks with \textbf{27} art movements. \textcolor{red}{The stylegan results are from the Munch trained stylegan model. We're in process of getting these features.}}
\label{tab:wiki_quant}
\end{table}

==> tables/observation_tables/wikiart_subset_quant_4k_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc|cc|cc}
\multicolumn{2}{c|}{{\color[HTML]{000000} }}                                                                          & \multicolumn{2}{c|}{{\color[HTML]{000000} \textbf{ARI}}}                                                                         & \multicolumn{2}{c}{{\color[HTML]{000000} \textbf{NMI}}}                                                                          \\ \cline{3-6} 
\multicolumn{2}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} \textbf{Features}}}}                                       & \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}}              & {\color[HTML]{000000} \textbf{DEC}}                  & \multicolumn{1}{c|}{{\color[HTML]{000000} \textbf{K-Means}}}              & {\color[HTML]{000000} \textbf{DEC}}                  \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{dense}$}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.007}}                         & {\color[HTML]{000000} 0.024}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.152}}                         & {\color[HTML]{000000} 0.167}                         \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{gram}$}      & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.051}}                         & {\color[HTML]{000000} 0.077}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.191}}                         & \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.251} \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{CNN}$}}}      & {\color[HTML]{000000} $F_{g \cdot c}$} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.01}}                          & {\color[HTML]{000000} 0.009}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.069}}                         & {\color[HTML]{000000} 0.067}                         \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{wvec}$}      & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.046}}                         & {\color[HTML]{000000} 0.049}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.152}}                         & {\color[HTML]{000000} 0.145}                         \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{coarse}$}    & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.001}}                         & {\color[HTML]{000000} 0.001}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.033}}                         & {\color[HTML]{000000} 0.033}                         \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{middle}$}    & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.001}}                         & {\color[HTML]{000000} 0.001}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.032}}                         & {\color[HTML]{000000} 0.03}                          \\
\multicolumn{1}{c|}{\multirow{-4}{*}{{\color[HTML]{000000} $F_{stylegan}$}}} & {\color[HTML]{000000} $F_{fine}$}      & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.001}}                         & {\color[HTML]{000000} 0.001}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.031}}                         & {\color[HTML]{000000} 0.032}                         \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{caption}$}   & \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.123}} & \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.136} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.326}} & \cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.32}  \\
\multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{000000} $F_{text}$}}}     & {\color[HTML]{000000} $F_{annot}$}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.095}}                         & \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.095} & \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.284}} & \cellcolor[HTML]{C0F1C8}{\color[HTML]{000000} 0.268} \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{stytr2}$}    & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.029}}                         & {\color[HTML]{000000} 0.033}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.131}}                         & {\color[HTML]{000000} 0.122}                         \\
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                                 & {\color[HTML]{000000} $F_{mamba}$}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.053}}                         & {\color[HTML]{000000} 0.075}                         & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.185}}                         & {\color[HTML]{000000} 0.198}                         \\
\multicolumn{1}{c|}{\multirow{-3}{*}{{\color[HTML]{000000} $F_{st}$}}}       & {\color[HTML]{000000} $F_{styleshot}$} & \multicolumn{1}{c|}{\cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.103}} & \cellcolor[HTML]{CAEDFB}{\color[HTML]{000000} 0.087} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.248}}                         & {\color[HTML]{000000} 0.23}                          \\ \hline
\multicolumn{1}{c|}{{\color[HTML]{000000} $F_{artist}$}}                     & {\color[HTML]{000000} $F_{CSD}$}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.25}}  & {\color[HTML]{000000} }                              & \multicolumn{1}{c|}{\cellcolor[HTML]{F2CEEF}{\color[HTML]{000000} 0.47}}  & {\color[HTML]{000000} }                             
\end{tabular}%
}
\caption{Metrics scores for the \textbf{WikiArt subset} dataset for all features for both K-Means and DEC model. The \colorbox[HTML]{F2CEEF}{best}, \colorbox[HTML]{C0F1C8}{second best} and the \colorbox[HTML]{CAEDFB}{third best} results are highlighted for each metric. The WikiArt subset dataset contains \textbf{4085} artworks with \textbf{27} art movements. The range of values for each metric are as follows: \textit{ARI}: -1 to 1, \textit{NMI}: 0 to 1.}
\label{tab:wiki_quant_4k}
\end{table}

==> tables/principles_of_art.tex <==
\begin{table}[]
%\captionsetup{justification=centering, labelsep=newline}
\resizebox{\hsize}{!}{
\begin{tabular}{l|l}
\textbf{Visual Elements} & \textbf{Concepts} \\ \hline
Subject & Representational, Non-representational \\ \hline
Line & \begin{tabular}[c]{@{}l@{}}Blurred, Broken, Controlled, Curved, Diagonal,\\ Horizontal, Vertical, Meandering, Thick, Thin, \\Active, Energetic, Straight\end{tabular} \\ \hline
Texture & Bumpy, Flat, Smooth, Gestural, Rough \\ \hline
 Color & \begin{tabular}[c]{@{}l@{}}
 Calm, Cool, Chromatic, Monochromatic, Muted,\\ Warm, Transparent \end{tabular} \\ \hline
Shape & \begin{tabular}[c]{@{}l@{}}Ambiguous, Geometric, Amorphous, Biomorphic,\\ Closed, Open, Distorted, Heavy, Linear, Organic, \\Abstract, Decorative, Kinetic, Light\end{tabular} \\ \hline
Light and Space & \begin{tabular}[c]{@{}l@{}}Bright, Dark, Medium, Atmospheric, Planar,\\ Perspective\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}General Principles \\of Art \end{tabular} & \begin{tabular}[c]{@{}l@{}}Overlapping, Balance, Contrast, Harmony, Pattern,\\ Repetition, Rhythm, Unity, Variety, Symmetry,\\ Proportion, Parallel\end{tabular}
\end{tabular}}
\caption{Visual elements and style concepts from \cite{8334453}.}
\label{tab: principles}
\end{table}
